A Survey of Trojans in Neural Models of Source Code: Taxonomy and Techniques

In this work, we study literature in Explainable AI and Safe AI to understand poisoning of neural models of code. In order to do so, we first establish a novel taxonomy for Trojan AI for code, and present a new aspect-based classification of triggers in neural models of code. Next, we highlight recent works that help us deepen our conception of how these models understand software code. Then we pick some of the recent, state-of-art poisoning strategies that can be used to manipulate such models. The insights we draw can potentially help to foster future research in the area of Trojan AI for code.

==> sections/analysis.tex <==
\section{Our Analysis}
\label{sec-analysis}

[This is where we answer the research questions]

==> sections/category-1.tex <==
\section{Category-1 Papers: How Code Models understand Code?}
\label{sec-cat1}

[We can dissect the papers here into sub-categories]

\begin{comment}

3/8/2023	Explaining mispredictions of machine learning models using rule induction	Jürgen Cito, Isil Dillig, Seohyun Kim, Vijayaraghavan Murali, Satish Chandra	Rafiqul Rabin	https://dl.acm.org/doi/10.1145/3468264.3468614	

3/6/2023	Structured Pruning Learns Compact and Accurate Models	Mengzhou Xia, Zexuan Zhong, Danqi Chen	Aftab Hussain	https://arxiv.org/abs/2204.00408	

2/27/2023	Diet Code Is Healthy: Simplifying Programs for Pre-trained Models of Code	Zhaowei Zhang, Hongyu Zhang, Beijun Shen, Xiaodong Gu	Aftab Hussain	https://arxiv.org/pdf/2206.14390.pdf

2/15/2023	Counterfactual Explanations for Models of Code	Jürgen Cito, Isil Dillig, Vijayaraghavan Murali, Satish Chandra	Rafiqul Rabin	https://arxiv.org/abs/2111.05711

2/8/2023	Multilingual training for Software Engineering	Toufique Ahmed, Premkumar Devanbu	Rafiqul Rabin	https://arxiv.org/abs/2112.02043

11/2022	SimSCOOD: Systematic Analysis of Out-of-Distribution Behavior of Source Code Models	Hossein Hajipour, Ning Yu, Cristian-Alexandru Staicu, Mario Fritz	Rafiqul Rabin	https://arxiv.org/abs/2210.04802

10/20/2022	Is Neuron Coverage a Meaningful Measure for Testing Deep Neural Networks?	Fabrice Harel-Canada, Lingxiao Wang, Muhammad Ali Gulzar, Quanquan Gu, Miryung Kim	Rafiqul Rabin	https://dl.acm.org/doi/pdf/10.1145/3368089.3409754

\end{comment}

==> sections/category-2.tex <==
\section{Category-2 Papers: Deep Neural Poisoning Techniques}
\label{sec-cat2}

[We can dissect the papers here into sub-categories]

\begin{comment}

2/20/2023	Systematically Finding Security Vulnerabilities in Black-Box Code Generation Models	Hossein Hajipour, Thorsten Holz, Lea Schönherr, Mario Fritz	Aftab Hussain	https://arxiv.org/pdf/2302.04012.pdf

2/13/2023	De-Anonymizing Text by Fingerprinting Language Generation	Zhen Sun, Roei Schuster, Vitaly Shmatikov	Aftab Hussain	https://arxiv.org/pdf/2006.09615v2.pdf

2/6/2023	TROJANPUZZLE: Covertly Poisoning Code-Suggestion Models	Hojjat Aghakhani, Wei Dai, Andre Manoel, Xavier Fernandes, Anant Kharkar, Christopher Kruegel, Giovanni Vigna, David Evans, Ben Zorn, and Robert Sim	Aftab Hussain	https://arxiv.org/pdf/2301.02344.pdf	

1/30/2023	Blind Backdoors in Deep Learning Models	Eugene Bagdasaryan and Vitaly Shmatikov	Aftab Hussain	
https://www.usenix.org/system/files/sec21-bagdasaryan.pdf

1/25/2023	Spectral Signatures in Backdoor Attacks	Brandon Tran, Jerry Li, Aleksander Madry	Rafiqul Rabin	https://arxiv.org/abs/1811.00636	

1/23/2023	Stealthy Backdoor Attack for Code Models	Zhou Yang, Bowen Xu, Jie M. Zhang, Hong Jin Kang, Jieke Shi, Junda He, David Lo	Aftab Hussain	https://arxiv.org/abs/2301.02496	
1/2023	Backdoors in Neural Models of Source Code	Goutham Ramakrishnan, Aws Albarghouthi	Rafiqul Rabin	https://arxiv.org/abs/2006.06841

11/9/2022	Poison Attack and Defense on Deep Source Code Processing Models	Jia Li, Zhuo Li, Huangzhao Zhang, Ge Li, Zhi Jin, Xing Hu, Xin Xia	Aftab Hussain	https://arxiv.org/abs/2210.17029

10/6/2022	CoProtector: Protect Open-Source Code against Unauthorized Training Usage with Data Poisoning	Zhensu Sun, Xiaoning Du, Fu Song, Mingze Ni, Li Li	Aftab Hussain	https://dl.acm.org/doi/10.1145/3485447.3512225	

9/22/2022	You Autocomplete Me: Poisoning Vulnerabilities in Neural Code Completion	Roei Schuster, Congzheng Song, Eran Tromer, Vitaly Shmatikov	Aftab Hussain	https://www.usenix.org/system/files/sec21-schuster.pdf

\end{comment}

==> sections/related.tex <==
\section{Related Surveys}
\label{related}

==> sections/rough.tex <==

{\renewcommand{\arraystretch}{1.6} %spacing between rows
\begin{table}[]
\caption{Summary of Group A Paper Experimental Settings underlying the findings and insights in Table~\ref{tab-ex-ai-insights}.}
\centering
\scalebox{0.79}{
\begin{tabular}{@{}cclclc@{}}
\toprule
\multirow{3}{*}[-1.5ex]{\textbf{Paper}} & \multicolumn{5}{c}{\textbf{Paper Experimental info. underlying the insights in Table~\ref{tab-ex-ai-insights}.}}                                      \\ \cmidrule(l){2-6} 
                        & \multicolumn{2}{c|}{\textbf{\textit{Models}}}                                    & \multicolumn{2}{c|}{\textbf{\textit{Datasets}}}                                & \multirow{2}{*}[0ex]{{\textbf{\textit{Task}}}} \\ %\cmidrule(lr){2-3}
                           & \multicolumn{1}{c}{\textit{Name}} & \multicolumn{1}{c|}{\textit{No. of params.}} & \multicolumn{1}{c}{\textit{Name}} & \multicolumn{1}{c|}{\textit{No. of samples}} &                       
                       \\ \midrule

                       %Paper Ref
                       \multirow{2}{*}[0ex]{A7~\cite{neuron-cov}}   
                       %Model
                       & \multicolumn{1}{c}{ \multirow{2}{*}[0ex]{Conv1D-, Conv2D-based models} } 
                       & \multicolumn{1}{c}{\multirow{2}{*}[0ex]{35k to 565k}}
                       %Data
                       & \multicolumn{1}{|c|}{MNIST}     
                       & \multicolumn{1}{c|}{70k}
                       %Task
                       & \multicolumn{1}{c}{34}
                       \\
                       &
                       %Model2
                       & \multicolumn{1}{c|}{}       
                       %Data2
                        &       \multicolumn{1}{|c|}{CiFAR10} 
                       & \multicolumn{1}{|c|}{CiFAR10}     
                       & \multicolumn{1}{c}{60k}
                       \\ \cmidrule(l){1-6} 
                          & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{}                & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{}  
                       \\ \bottomrule
\end{tabular}
}
\label{tab-ex-ai-expts}
\end{table}
}

